Maxmin Participatory Budgeting

Participatory Budgeting (PB) is a popular voting method by which a limited budget is divided among a set of projects, based on the preferences of voters over the projects. PB is broadly categorised as divisible PB (if the projects are fractionally implementable) and indivisible PB (if the projects are atomic). Egalitarianism, an important objective in PB, has not received much attention in the context of indivisible PB. This paper addresses this gap through a detailed study of a natural egalitarian rule, Maxmin Participatory Budgeting (MPB), in the context of indivisible PB. Our study is in two parts: (1) computational (2) axiomatic. In the first part, we prove that MPB is computationally hard and give pseudo-polynomial time and polynomial-time algorithms when parameterized by certain well-motivated parameters. We propose an algorithm that achieves for MPB, additive approximation guarantees for restricted spaces of instances and empirically show that our algorithm in fact gives exact optimal solutions on real-world PB datasets. We also establish an upper bound on the approximation ratio achievable for MPB by the family of exhaustive strategy-proof PB algorithms. In the second part, we undertake an axiomatic study of the MPB rule by generalizing known axioms in the literature. Our study leads to the proposal of a new axiom, maximal coverage, which captures fairness aspects. We prove that MPB satisfies maximal coverage.

==> header.tex <==
%%PACKAGES%%
\usepackage{xspace}
%\usepackage{amssymb}
\usepackage{mathtools}
%to drawrules like toprule, midrule
\usepackage[capitalise]{cleveref} %references will include the types
\usepackage[hidelinks]{hyperref}
\RequirePackage{comment}
\usepackage{xifthen}
\usepackage{arydshln}
\usepackage{xcolor}
\usepackage{amssymb}
\usepackage{dsfont}
%\usepackage[linesnumbered,ruled,vlined]{algorithm2e}
\usepackage{bbm}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{colortbl}
\usepackage{graphics}
\usepackage{float}
\usepackage{color}
\usepackage{xcolor}
\usepackage{array}
\usepackage{multirow}
\usepackage{enumitem}
\usepackage{tikz}
\usepackage{xifthen}
\makeatletter
\newcommand{\setword}[2]{%
  \phantomsection
  #1\def\@currentlabel{\unexpanded{#1}}\label{#2}%
}
\makeatother
\usepackage{atbegshi,etoolbox}% http://ctan.org/pkg/{lipsum,atbegshi,etoolbox}
\makeatletter
\newcommand{\discardpages}[1]{% \discardpages{<csv list>}
  \xdef\discard@pages{#1}% Store pages to discard
  \AtBeginShipout{% At shipout, decide whether to discard page/not
    \renewcommand*{\do}[1]{% How to handle each page entry in csv list
      \ifnum\value{page}=##1\relax%
        \AtBeginShipoutDiscard% Discard page/not
        \gdef\do####1{}% Do nothing further
      \fi%
    }%
    \expandafter\docsvlist\expandafter{\discard@pages}% Process list of pages to discard
  }%
}

%%FOR MATHCAL%%
\renewcommand{\AA}{\ensuremath{\mathcal A}\xspace}
\newcommand{\BB}{\ensuremath{\mathcal B}\xspace}
\newcommand{\CC}{\ensuremath{\mathcal C}\xspace}
\newcommand{\DD}{\ensuremath{\mathcal D}\xspace}
\newcommand{\EE}{\ensuremath{\mathcal E}\xspace}
\newcommand{\FF}{\ensuremath{\mathcal F}\xspace}
\newcommand{\GG}{\ensuremath{\mathcal G}\xspace}
\newcommand{\HH}{\ensuremath{\mathcal H}\xspace}
\newcommand{\II}{\ensuremath{\mathcal I}\xspace}
\newcommand{\JJ}{\ensuremath{\mathcal J}\xspace}
\newcommand{\KK}{\ensuremath{\mathcal K}\xspace}
\newcommand{\LL}{\ensuremath{\mathcal L}\xspace}
\newcommand{\MM}{\ensuremath{\mathcal M}\xspace}
\newcommand{\NN}{\ensuremath{\mathcal N}\xspace}
\newcommand{\OO}{\ensuremath{\mathcal O}\xspace}
\newcommand{\PP}{\ensuremath{\mathcal P}\xspace}
\newcommand{\QQ}{\ensuremath{\mathcal Q}\xspace}
\newcommand{\RR}{\ensuremath{\mathcal R}\xspace}
\renewcommand{\SS}{\ensuremath{\mathcal S}\xspace}
\newcommand{\TT}{\ensuremath{\mathcal T}\xspace}
\newcommand{\UU}{\ensuremath{\mathcal U}\xspace}
\newcommand{\VV}{\ensuremath{\mathcal V}\xspace}
\newcommand{\WW}{\ensuremath{\mathcal W}\xspace}
\newcommand{\XX}{\ensuremath{\mathcal X}\xspace}
\newcommand{\YY}{\ensuremath{\mathcal Y}\xspace}
\newcommand{\ZZ}{\ensuremath{\mathcal Z}\xspace}

%%FOR MATH FRAK%%
\newcommand{\aaa}{\ensuremath{\mathfrak a}\xspace}
\newcommand{\bbb}{\ensuremath{\mathfrak b}\xspace}
\newcommand{\ccc}{\ensuremath{\mathfrak c}\xspace}
\newcommand{\ddd}{\ensuremath{\mathfrak d}\xspace}
\newcommand{\eee}{\ensuremath{\mathfrak e}\xspace}
\newcommand{\fff}{\ensuremath{\mathfrak f}\xspace}
%\newcommand{\ggg}{\ensuremath{\mathfrak g}\xspace}
%\newcommand{\hhh}{\ensuremath{\mathfrak h}\xspace}
\newcommand{\iii}{\ensuremath{\mathfrak i}\xspace}
\newcommand{\jjj}{\ensuremath{\mathfrak j}\xspace}
\newcommand{\kkk}{\ensuremath{\mathfrak k}\xspace}
%\newcommand{\lll}{\ensuremath{\mathfrak l}\xspace}
\newcommand{\mmm}{\ensuremath{\mathfrak m}\xspace}
\newcommand{\nnn}{\ensuremath{\mathfrak n}\xspace}
\newcommand{\ooo}{\ensuremath{\mathfrak o}\xspace}
\newcommand{\ppp}{\ensuremath{\mathfrak p}\xspace}
\newcommand{\qqq}{\ensuremath{\mathfrak q}\xspace}
\newcommand{\rrr}{\ensuremath{\mathfrak r}\xspace}
\newcommand{\sss}{\ensuremath{\mathfrak s}\xspace}
\newcommand{\ttt}{\ensuremath{\mathfrak t}\xspace}
\newcommand{\uuu}{\ensuremath{\mathfrak u}\xspace}
\newcommand{\vvv}{\ensuremath{\mathfrak v}\xspace}
\newcommand{\www}{\ensuremath{\mathfrak w}\xspace}
\newcommand{\xxx}{\ensuremath{\mathfrak x}\xspace}
\newcommand{\yyy}{\ensuremath{\mathfrak y}\xspace}
\newcommand{\zzz}{\ensuremath{\mathfrak z}\xspace}

%%FOR THEOREMS ETC.%%
\newtheorem{proposition}{\bf Proposition}
\newtheorem{observation}{\bf Observation}
%\newtheorem{theorem}{\bf Theorem}
\newtheorem{lemma}{\bf Lemma}
\newtheorem{corollary}{\bf Corollary}
\newtheorem{definition}{\bf Definition}
\newtheorem{claim}{\bf Claim}
\newtheorem{reductionrule}{\bf Reduction rule}
\crefname{theorem}{theorem}{\bf Theorem}
\crefname{example}{example}{\bf Example}
\crefname{observation}{observation}{\bf Observation}
\crefname{lemma}{lemma}{\bf Lemma}
\crefname{corollary}{corollary}{\bf Corollary}
\crefname{proposition}{proposition}{\bf Proposition}
\crefname{definition}{definition}{\bf Definition}
\crefname{claim}{claim}{\bf Claim}
\crefname{reductionrule}{reduction rule}{\bf Reduction rule}

%%FOR COMMON COMMANDS%%
\DeclareMathOperator*{\argmaxaa}{arg\,max}
\DeclareMathOperator*{\argminaa}{arg\,min}
\newcommand{\argmi}{\argminaa\limits_}
\newcommand{\argma}{\argmaxaa\limits_}
\newcommand{\instance}{\ensuremath{\mathcal{I}}\xspace}
\newcommand{\suml}{\sum\limits_}
\newcommand{\maxl}{\max\limits_}
\newcommand{\minl}{\min\limits_}
\newcommand{\lb}{\left(}
\newcommand{\rb}{\right)}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
\newcommand{\curly}[1]{\ensuremath{\{#1\}}\xspace}
\newcommand{\nn}{\nonumber}
\newcommand{\NPH}{\ensuremath{\mathsf{NP}}-hard\xspace}
\newcommand{\WH}{\ensuremath{\mathsf{W[1]}}-hard\xspace}
\newcommand{\WWH}{\ensuremath{\mathsf{W[2]}}-hard\xspace}
\newcommand{\NP}{\ensuremath{\mathsf{NP}}\xspace}
\newcommand{\NPC}{\ensuremath{\mathsf{NP}}-complete\xspace}
\newcommand{\subsum}{{\sc Subset Sum}\xspace}
\newcommand{\egalbloc}{{\sc Egalitarian-Bloc}\xspace}
\newcommand{\vercov}{{\sc Vertex Cover}\xspace}
\newcommand{\setcov}{{\sc Set Cover}\xspace}
\newcommand{\knap}{{\sc Knapsack}\xspace}
\newcommand{\ccmw}{{\sc $\beta$-CC}\xspace}
\newcommand{\yes}{{\sc Yes}\xspace}
\newcommand{\no}{{\sc No}\xspace}
\newcommand{\FPT}{\ensuremath{\mathsf{FPT}}\xspace}

%%FOR NEW COMMANDS CUSTOMISED FOR THE PAPER%%
\newcommand{\bud}{\ensuremath{b}\xspace}
\newcommand{\proj}{\ensuremath{P}\xspace}
\newcommand{\voters}{\ensuremath{N}\xspace}
\newcommand{\feasible}{\ensuremath{\mathcal{E}}\xspace}
%\newcommand{\exhaustive}{\ensuremath{\mathcal{E}}\xspace}
\newcommand{\prof}{\ensuremath{\mathcal{A}}\xspace}
\newcommand{\ii}{\ensuremath{i}\xspace}
\newcommand{\jj}{\ensuremath{j}\xspace}
\newcommand{\pp}{\ensuremath{p}\xspace}
\newcommand{\pa}{\ensuremath{a}\xspace}
\newcommand{\distinct}{\ensuremath{\hat{n}}\xspace}
\newcommand{\scalel}{\ensuremath{\delta}\xspace}
%\newcommand{\ov}{\Theta}
\newcommand{\weakhcbp}{weak-\ensuremath{\mathsf{HCBP}}\xspace}
\newcommand{\stronghcbp}{strong-\ensuremath{\mathsf{HCBP}}\xspace}
\newcommand{\hcbp}{\ensuremath{\mathsf{HCBP}}\xspace}
\newcommand{\mmpb}{\ensuremath{\mathsf{MPB}}\xspace}
\newcommand{\MAV}{\ensuremath{\mathsf{MAV}}\xspace}
\newcommand{\lpalgo}{{\sc Ordered-Relax}\xspace}
\newcommand{\real}{\mathbb{R}_{\geq 0}}
\newcommand{\optset}{\ensuremath{O}\xspace}
\newcommand{\opt}{\emph{OPT}}
\newcommand{\alg}{\emph{ALG}}
\newcommand{\lo}{\ensuremath{l_o}\xspace}
\newcommand{\ho}{\ensuremath{h_o}\xspace}
\newcommand{\la}{\ensuremath{l_{\prof}}\xspace}
\newcommand{\ha}{\ensuremath{h_{\prof}}\xspace}
%\newcommand{\caxas}{c(a)x_a^*}
%\newcommand{\cbxbs}{c(b)x_b^*}
%\newcommand{\caxa}{c(a)x_a}
\newcommand{\aof}[1]{%
  \ifthenelse{\isempty{#1}}%
    {\ensuremath{A_i}\xspace}% if #1 is empty
    {\ensuremath{A_{#1}}\xspace}% if #1 is not empty
}
\newcommand{\bool}{\ensuremath{\mathds{1}}}
\newcommand{\uof}[2]{%
  \ifthenelse{\isempty{#1}}%
    {\ensuremath{\operatorname{u_i\!}\left(#2\right)}\xspace}% if #1 is empty
    {\ensuremath{\operatorname{u_{#1}\!}\left(#2\right)}\xspace}% if #1 is not empty
}
\newcommand{\disuof}[2]{%
  \ifthenelse{\isempty{#1}}%
    {\ensuremath{\operatorname{d_i\!}\left(#2\right)}\xspace}% if #1 is empty
    {\ensuremath{\operatorname{d_{#1}\!}\left(#2\right)}\xspace}% if #1 is not empty
}
\newcommand{\fdisuof}[2]{%
  \ifthenelse{\isempty{#1}}%
    {\ensuremath{\bud-{\uof{}{#2}}}\xspace}% if #1 is empty
    {\ensuremath{\bud-{\uof{#1}{#2}}}\xspace}% if #1 is not empty
}
\newcommand{\cof}[1]{\ensuremath{\operatorname{c\!}\left(#1\right)}\xspace}
\newcommand{\cxof}[1]{\ensuremath{\operatorname{c\!}\left(#1\right)x_{#1}}\xspace}
\newcommand{\cdxof}[1]{\ensuremath{\operatorname{c}'\!\left(#1\right)x_{#1}}\xspace}
\newcommand{\cxsof}[1]{\ensuremath{\operatorname{c\!}\left(#1\right)x_{#1}^*}\xspace}
\newcommand{\br}{\ensuremath{R}\xspace}
\newcommand{\mmpbr}{\ensuremath{M}\xspace}
\newcommand{\winnerfunction}{\ensuremath{\mathcal{W}}\xspace}
\newcommand{\ruleof}[2]{%
  \ifthenelse{\isempty{#2}}%
    {\ensuremath{\operatorname{#1\!}\left(\instance\right)}\xspace}% if #2 is empty
    {\ensuremath{\operatorname{#1\!}\left(\instance#2\right)}\xspace}% if #2 is not empty
}
\newcommand{\winners}[2]{%
  \ifthenelse{\isempty{#2}}%
    {\ensuremath{\operatorname{\winnerfunction_{#1}\!}\left(\instance\right)}\xspace}% if #2 is empty
    {\ensuremath{\operatorname{\winnerfunction_{#1}\!}\left(\instance#2\right)}\xspace}% if #2 is not empty
}
\newcommand{\fullinstance}{\ensuremath{\langle \voters,\proj,c,\bud,\prof \rangle}\xspace}
\newcommand{\firstfrac}[1]{%
  \ifthenelse{\isempty{#1}}%
    {\ensuremath{\frac{|S|-|Y_i|}{|\aof{}|-|Y_i|}}\xspace}% if #1 is empty
    {\ensuremath{\frac{|S|-|Y_{#1}|}{|\aof{#1}|-|Y_{#1}|}}\xspace}% if #1 is not empty
}
\newcommand{\revfrac}[1]{%
  \ifthenelse{\isempty{#1}}%
    {\ensuremath{\frac{|S|-|\aof{}|}{|S|-|Y_i|}}\xspace}% if #1 is empty
    {\ensuremath{\frac{|S|-|\aof{#1}|}{|S|-|Y_{#1}|}}\xspace}% if #1 is not empty
}
\newcommand{\frack}[1]{%
  \ifthenelse{\isempty{#1}}%
    {\ensuremath{\frac{|\aof{}|-|Y_i|}{|S|-|Y_i|}}\xspace}% if #1 is empty
    {\ensuremath{\frac{|\aof{#1}|-|Y_{#1}|}{|S|-|Y_{#1}|}}\xspace}% if #1 is not empty
}
\newcommand{\longversion}{\cite{aziz2018rank}}
\newcommand{\longversionshort}{Sreedurga et al. \shortcite{aziz2018rank}}
\newcommand{\githublink}{\url{https://github.com/Participatory-Budgeting/maxmin_2022}}
